Knowledge Distillation: Bad Models Can Be Good Role Models

Large neural networks trained in the overparameterized regime are able to fit noise to zero train error. Recent work \citep{nakkiran2020distributional} has empirically observed that such networks behave as "conditional samplers" from the noisy distribution. That is, they replicate the noise in the train data to unseen examples. We give a theoretical framework for studying this conditional sampling behavior in the context of learning theory. We relate the notion of such samplers to knowledge distillation, where a student network imitates the outputs of a teacher on unlabeled data. We show that samplers, while being bad classifiers, can be good teachers. Concretely, we prove that distillation from samplers is guaranteed to produce a student which approximates the Bayes optimal classifier. Finally, we show that some common learning algorithms (e.g., Nearest-Neighbours and Kernel Machines) can generate samplers when applied in the overparameterized regime.

==> sections/intro.tex <==
\section{Introduction}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.31\textwidth]{figures/noisy-cifar10.pdf} \hfil 
    \includegraphics[width=0.34\textwidth]{figures/ensemble-cifar10.pdf} \hfil 
    \includegraphics[width=0.32\textwidth]{figures/random-cifar10.pdf}\hfil
    \caption{\textbf{From Samplers to Good Models.}  Class confusion matrices for ResNet-18 trained on CIFAR-10 with 20\% fixed and class dependent label noise (e.g., 20\% of cats are labeled as dogs). \emph{Left.} A standalone ResNet-18 trained on this data \emph{replicates} the noise to the test distribution. \emph{Middle.} When ensembling 10 such models, the noise virtually disappears, however incurring a high price at inference. \emph{Right.} Distilling a single model via unlabeled examples from the CIFAR-5m dataset using a randomly selected teacher from a pool of 10 such teachers  for each example eliminates the noise as well as the inference cost.
    }
    \label{fig:intro}
\end{figure*}

\todo{consider putting the next section as part of the introduction}
Neural networks with a large number of parameters are often trained in the over-parameterized regime, where there are much more parameters than labeled examples. In this regime, it has been shown empirically and theoretically \todo{cite} that neural networks are capable of fitting the training data to zero loss, even when the labels are noisy (or, in the extreme case, when the labels are complete noise). Recently, in a work by \cite{nakkiran2020distributional}, it has been observed empirically that neural networks tend to replicate the noise of the training data to unseen (test) data as well. For example, given an image classification task, if 30\% of the dogs are mislabeled as cats, the trained model will label approximately 30\% of the dogs \textit{in the test data} as cats. In this sense, deep networks behave very similarly to the 1-Nearest-Neighbour rule over some representation of the input. \todo{this might be a good point to add a figure from preetum} In other words, neural networks behave like \textit{samplers} from the noisy distribution, where the prediction of the label $y$ for some example $\x$ follows a distribution that is similar to the distribution of $\P[y|\x]$ in the input distribution.

The observation that neural networks in the over-parameterized regime replicate the noise of the train data means that their performance degrades with the amount of noise. Since the goal in learning from noisy data is to approximate the ``correct'' labeling function (namely, the Bayes optimal prediction over the noisy distribution), \textit{samplers} from the data distributions make bad \textit{classifiers}.
However, in this work we show that \textit{samplers} can be used to label a new (and potentially larger) unlabeled dataset, which is then used to successfully train a \textit{student} classifier, in a process known as \textit{knowledge distillation}.
Indeed, knowledge distillation has become a very popular technique for achieving state-of-the-art performance on various tasks. Our results suggest a simple way to interpret the success of distillation, via the observation that noisy predictors can be bad \textit{classifiers} but good \textit{teachers}.

We now summarize the main contributions of our work. First, we relate the notion of \textit{samplers} introduced in \cite{nakkiran2020distributional} to knowledge distillation methods, showing that \textit{samplers} can be good \textit{teachers} (Section \ref{sec:setting}). Building on this, we show that by distillation from an ensemble of \textit{samplers}, one can get a student that achieves low error w.r.t. the \textit{clean} distribution (i.e., approximating the Bayes optimal prediction).
Our theoretical framework leads to a new distillation method, where instead of using the ensemble to generate labels we randomly pick a single classifier from a fixed set of classifiers for labeling each example. This method has computational benefits over using the ensemble, and to the best of our knowledge it was not introduced in prior work. We prove that this new technique can also yield a student with low error. Both distillation methods are analyzed in Section \ref{sec:distillation}. In Section \ref{sec:algorithms}, we show that some well-known algorithms, such as k-Nearest-Neighbour, kernel methods and  neural networks are samplers or teachers in some setting. This partly solves some conjectures raised in \cite{nakkiran2020distributional}\todo{does it?}. Finally, in Section \ref{sec:experiments} we complement our theoretical findings with experiments, showing that the distillation methods studied in this work improve the performance of neural networks when training on noisy data.
\todo{EM: among other things, let's discuss literature on learning from noisy data, and say that unlike many works we don't assume the noise is i.i.d.}

